Verisig: verifying safety properties of hybrid systems with neural network controllers

This paper presents Verisig, a hybrid system approach to verifying safety properties of closed-loop systems using neural networks as controllers. Although techniques exist for verifying input/output properties of the neural network itself, these methods cannot be used to verify properties of the closed-loop system (since they work with piecewise-linear constraints that do not capture non-linear plant dynamics). To overcome this challenge, we focus on sigmoid-based networks and exploit the fact that the sigmoid is the solution to a quadratic differential equation, which allows us to transform the neural network into an equivalent hybrid system. By composing the network's hybrid system with the plant's, we transform the problem into a hybrid system verification problem which can be solved using state-of-the-art reachability tools. We show that reachability is decidable for networks with one hidden layer and decidable for general networks if Schanuel's conjecture is true. We evaluate the applicability and scalability of Verisig in two case studies, one from reinforcement learning and one in which the neural network is used to approximate a model predictive controller.

==> temp.tex <==
%!TEX root = main.tex

\section{Case Study Applications}
\label{sec:results}
This section presents two case studies in order to illustrate possible
use cases for the proposed verification approach. These case studies
were chosen in domains where DNNs are used extensively as controllers,
with weak worst-case guarantees about the trained network; this means
it is essential to verify properties about these closed-loop systems
in order to assure their functionality. The first case study,
presented in Section~\ref{sec:rl}, is Mountain Car, a benchmark
problem in RL. Section~\ref{sec:mpc_dnn} presents the second case
study in which a DNN is used to approximate an MPC with safety
guarantees.

\begin{figure}[!t]
  \centering 
  \includegraphics[width=0.8\linewidth]{fig/Mcar}
  \caption{Mountain Car problem~\cite{openaigym}. The car needs to
    drive up the left hill first in order to gather enough momentum
    and reach its goal on the right.}
  \label{fig:Mcar}
\end{figure}

\subsection{Mountain Car: A Reinforcement Learning Case Study}
\label{sec:rl}
This subsection illustrates how Verisig could be used to verify
properties on a benchmark deep RL problem, namely Mountain
Car. Mountain Car (MC) is a problem in which an under-powered car must
drive up a steep hill, shown in Figure~\ref{fig:Mcar}. Since the car
does not have enough power to simply accelerate up the hill, it needs
to drive up the opposite hill first in order to gather enough momentum
so as to be able to reach its goal. The learning task is to learn a
controller that takes as input the car's position and velocity and
outputs an acceleration command. In this paper, we consider the
continuous version of the problem such that acceleration is a real
number between -1 and 1 (negative inputs mean acceleration to the
left). Given input acceleration at time $k$, denoted by $u_k$, the car
dynamics are described the following non-linear system:
%
\begin{align*}
p_{k+1} &= p_k + v_{k}\\
v_{k+1} &= v_k + 0.0015u_k - 0.0025*cos(3p_k),
\end{align*}
%
where $p_k$ and $v_k$ are the car's position and velocity,
respectively, with $p_0$ chosen uniformly at random from $[-0.6,
  -0.4]$ and $v_0 = 0$. Note that velocity is constrained to be within
$[-0.07, 0.07]$ and position is constrained to be within $[-1.2,
  0.6]$, thereby introducing (hybrid) mode switches when these
constraints are violated.

During the training stage, the training algorithm tries different
control actions and observes a reward; the goal of training is to
maximize the agent's reward. In MC, the reward associated with a
control action $a$ is $-0.1a^2$, i.e., larger acceleration values are
penalized more so as to avoid a ``bang-bang'' strategy. A reward of
100 is received when the car reaches its goal. The training stage
typically occurs over multiple episodes (if not solved, an episode is
terminated after 1000 steps) such that various behaviors can be
observed.  MC is considered ``solved'' if, during testing, the car
goes up the hill with an average reward of at least 90 over 100
consecutive trials.

We trained a DNN controller for MC within the environment provided by
OpenAI Gym~\cite{openaigym}, a toolkit for developing and comparing
algorithms on benchmark RL problems. We utilized a standard
actor/critic approach for deep RL problems~\cite{lillicrap15}. This is
a two-DNN setting in which one DNN (the critic) learns the reward
function, whereas the other one (the actor) learns the control. Once
training is finished, the actor is deployed as the DNN controller for
the closed-loop system. We trained a two-hidden-layer sigmoid-based
DNN with 16 neurons per layer; the last layer has a tanh activation
function in order to scale the output to be between -1 and 1. Note
that larger networks were also trained in order to evaluate
scalability, as discussed in Section~\ref{sec:comparison}.

Using Verisig, one can strengthen the definition of a ``solved'' task
and actually verify that the car will go up the hill with a reward of
at least 90 starting from \emph{any} initial condition. In order to
verify whether the closed-loop system using our trained DNN satisfies
this property, we transformed the DNN into an equivalent hybrid system
using the technique presented in Section~\ref{sec:approach} and
composed it with the hybrid system describing the car's dynamics. We
then used Flow* to verify whether the car will go up the hill with a
reward of at least 90, given any initial position in [-0.6,
  -0.4].

\begin{table}
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
Initial condition   & Verified  & Reward & \# steps & Time \\ \hline
[-0.41, -0.40] & Yes & >= 90  & <= 100  & 4277s  \\ \hline
[-0.415, -0.41] & Yes & >= 90  & <= 100  & 4729s  \\ \hline
[-0.43, -0.415] & Yes & >= 90  & <= 100  & 2324s  \\ \hline
[-0.45, -0.43] & Yes & >= 90  & <= 100  & 2091s  \\ \hline
[-0.48, -0.45] & Yes & >= 90  & <= 100  & 2018s  \\ \hline
[-0.50, -0.48] & Yes & >= 90  & <= 100  & 1866s  \\ \hline
[-0.55, -0.50] & Yes & >= 90  & <= 100  & 2272s  \\ \hline
[-0.57, -0.55] & Yes & >= 90  & <= 100  & 2057s  \\ \hline
[-0.59, -0.57] & Yes & >= 90  & <= 106  & 2494s  \\ \hline
[-0.6, -0.59] & No & N/A  & N/A  & N/A  \\ \hline
\end{tabular}
\caption{Verisig+Flow* verification times (in seconds) for different
  initial conditions of the Mountain Car problem. The third column
  shows the lower bound of reward that was verified. The fourth column
  shows the upper bound of the number of dynamics steps that was
  verified.}
\label{tab:mc}
\end{table}

Note that we split the initial condition into subsets and verified the
property for each subset separately. This was necessary because the
DNN took very different actions from different initial conditions,
e.g., large negative inputs when the car was started from the leftmost
position and small negative inputs when the car was started from the
rightmost position. This variability in turn introduced a lot of
uncertainty in the dynamics, and caused large approximation errors.

Table~\ref{tab:mc} presents the verification results in terms of the
time to verify the property for each subset. As can be seen in the
table, for each subset, Verisig took about 35 minutes to verify the
property (two properties took longer to verify due to branching in the
car's hybrid system as caused by the car reaching the minimum allowed
position). Indeed, for most initial conditions, we verified that the
car will go up the hill with a reward of at least 90 and in at most
100 dynamics steps. Interestingly, after failing to verify the
property for the last subset, [-0.6, -0.59], we found a
counter-example to the property when starting the car from $p_0 =
-0.6$: the final reward was 88. This suggests that Verisig is not only
useful in verifying properties of interest but it can also be used
identify areas for which these properties do not hold. In the case of
MC, this information can be used to retrain the DNN by starting more
episodes from [-0.6, -0.59] since the likely reason the DNN did not
perform well from that initial condition is that not many data points
were observed there during training.

\begin{figure}[!t]
  \centering 
  \includegraphics[width=1\linewidth]{fig/uncertainty}
  \caption{Verisig+Flow* approximation sets over time.}
  \label{fig:uncertainty}
\end{figure}

Finally, we illustrate the uncertainty of the approximation sets
created by Verisig+Flow* over time. Figure~\ref{fig:uncertainty} shows
a two-dimensional projection of the approximation sets over time (for
the case $p_0 \in [-0.5, -0.48]$), with the DNN control inputs plotted
on the x-axis and the car's position on the y-axis. Initially, the
uncertainty is fairly small and remains so until the car goes up the
left hill and starts going quickly downhill. At that point, the
uncertainty is relatively big but it still remains within the
tolerance necessary to verify the desired property.

\subsection{Using DNNs to Approximate MPCs with Safety Guarantees}
\label{sec:mpc_dnn}
To further evaluate the applicability of Verisig, in this subsection
we consider a different case study, in which a DNN is used to
approximate an MPC with safety guarantees. DNNs have recently been
used to approximate controllers for different reasons: 1) the MPC
computation is not fast enough so as to be feasible at
run-time~\cite{hertneck18}; 2) storing the controller (e.g., as a
lookup table) requires too much memory~\cite{julian16}; 3) performing
reachability analysis is infeasible for high-dimensional systems by
discretizing the state space~\cite{royo18}. In this paper, we focus on
the latter scenario in which the aim is to develop a DNN controller
with safety guarantees.

As described in prior work~\cite{royo18}, it is possible to train a
DNN approximating an MPC in the case of control-affine systems
following a piecewise-linear high-level planner. In such a case, the
optimal control strategy is ``bang-bang'', i.e., the controller is
effectively a classifier mapping a system state to one of finitely
many control actions. Once the DNN is trained, one can simulate the
closed-loop system over a finite horizon $T$ with a worst-case planner
(which also follows a ``bang-bang'' strategy) -- the largest deviation
from the planner is a worst-case guarantee for the deviation from
\emph{any} other plan over horizon $T$. Thus, it is possible to obtain
safety guarantees for the system assuming that it always start from
the same initial condition.

\begin{figure}[!t]
  \centering 
  \includegraphics[width=0.8\linewidth]{fig/quad_cs}
  \caption{Overview of the quadrotor case study, as projected to the
    $(x,y)$-plane. The quadrotor's goal is to follow its planner in
    order to reach the goal at the top (star) without colliding into
    obstacles (red circles). We have verified that, starting from any
    state within the shown set of initial conditions, the quadrotor
    will not deviate from its plan by more than 0.32m (and hence will
    not collide into any obstacles).}
  \label{fig:quad_cs}
\end{figure}

In this case study, we consider a six-dimensional control-affine
quadrotor controlled by a DNN and verify that the quadrotor, as
started from a set of initial conditions, will reach its goal without
colliding into nearby obstacles. Specifically, the quadrotor follows a
path planner, given as a piecewise-linear system, and tries to stay as
close to the planner as possible. The setup, as projected to the
$(x,y)$-plane, is shown in Figure~\ref{fig:quad_cs}. The quadrotor and
planner dynamics models are as follows:
%
\begin{align}
\label{eq:quad_model}
\dot{q} := \left[\begin{array}{c}
\dot{p}_x^q\\
\dot{p}_y^q\\
\dot{p}_z^q\\
\dot{v}_x^q\\
\dot{v}_y^q\\
\dot{v}_z^q\end{array}\right] = \left[\begin{array}{c}
v_x^q\\
v_y^q\\
v_z^q\\
g\text{tan}\theta\\
-g\text{tan}\phi\\
\tau - g\end{array}\right], \dot{p} := \left[\begin{array}{c}
\dot{p}_x^p\\
\dot{p}_y^p\\
\dot{p}_z^p\\
\dot{v}_x^p\\
\dot{v}_y^p\\
\dot{v}_z^p\end{array}\right] = \left[\begin{array}{c}
b_x\\
b_y\\
b_z\\
0\\
0\\
0\end{array}\right],
\end{align}
%
where $p_x^q, p_y^q, p_z^q$ and $p_x^p, p_y^p, p_z^p$ are the
quadrotor and the planner's positions in three dimensions,
respectively; $v_x^q, v_y^q, v_z^q$ and $v_x^p, v_y^p, v_z^p$ are the
quadrotor and the planner's velocities in three dimensions,
respectively; $\theta$, $\phi$ and $\tau$ are contol inputs (given as
pitch, roll and thrust); $g = 9.81 m/s^2$ is Earth's gravity; $b_x,
b_y, b_z$ are piecewise constant. The control inputs have the
constraints $\phi, \theta \in [-0.1, 0.1]$ and $\tau \in [7.81,
  11.81]$, whereas the planner velocities have constraints $b_x, b_y,
b_z \in [-0.25, 0.25]$. Thus, the controller's goal for this quadrotor
is to stabilize the system of relative states $r := [p_x^r, p_y^r,
  p_z^r, v_x^r, v_y^r, v_z^r]^{\top} = q - p$, i.e., ensure the
quadrotor is as close to the planner as possible.

To train a DNN controller for the model in~\eqref{eq:quad_model}, we
followed the approach described in prior work~\cite{royo18}. In
particular, we sample multiple points from the state space over a time
horizon $T$ and train a sequence of DNNs, one for each dynamics step
(the dynamics are discretized using the Runge-Kutta method). Once two
consecutive DNNs have similar training error, we interrupt the
training and pick the last DNN as the final controller. The DNN takes
a relative state as input and outputs one of eight possible actions
(recall that a ``bang-bang'' strategy means there are two options per
control action). For this case study, we trained a two-hidden layer
DNN, with 20 neurons per layer and tanh activations, and a linear last
layer.

Given the trained DNN controller, we verified a safety property for
the closed-loop system given the setup whose $(x,y)$-plane projection
is shown in Figure~\ref{fig:quad_cs}. Specifically, the quadrotor is
started from an initial condition $(p_x^r, p_y^r) \in [-0.05, -0.05]
\times [-0.05, -0.05]$ (the other states are initialized at 0) and
needs to stay within 0.32m from the planner in order to reach its goal
without colliding into obstacles.

\begin{table}
\centering
\begin{tabular}{|l|c|c|}
\hline
Initial condition on $(p_x^r, p_y^r)$  & Property & Time \\ \hline
$[-0.05, -0.025] \times [-0.05, -0.025]$ & $\|r_3\|_{\infty} \le 0.32m$ & 2766s  \\ \hline
$[-0.025, 0] \times [-0.05, -0.025]$ & $\|r_3\|_{\infty} \le 0.32m$ & 2136s  \\ \hline
$[0, 0.025] \times [-0.05, -0.025]$ & $\|r_3\|_{\infty} \le 0.32m$ & 2515s  \\ \hline
$[0.025, 0.05] \times [-0.05, -0.025]$ & $\|r_3\|_{\infty} \le 0.32m$ & 897s  \\ \hline
$[-0.05, -0.025] \times [-0.025, 0]$ & $\|r_3\|_{\infty} \le 0.32m$ & 1837s  \\ \hline
$[-0.025, 0] \times [-0.025, 0]$ & $\|r_3\|_{\infty} \le 0.32m$ & 1127s  \\ \hline
$[0, 0.025] \times [-0.025, 0]$ & $\|r_3\|_{\infty} \le 0.32m$ & 1593s  \\ \hline
$[0.025, 0.05] \times [-0.025, 0]$ & $\|r_3\|_{\infty} \le 0.32m$ & 894s  \\ \hline
$[-0.05, -0.025] \times [0, 0.025]$ & $\|r_3\|_{\infty} \le 0.32m$ & 1376s  \\ \hline
$[-0.025, 0] \times [0, 0.025]$ & $\|r_3\|_{\infty} \le 0.32m$ & 953s  \\ \hline
$[0, 0.025] \times [0, 0.025]$ & $\|r_3\|_{\infty} \le 0.32m$ & 1038s  \\ \hline
$[0.025, 0.05] \times [0, 0.025]$ & $\|r_3\|_{\infty} \le 0.32m$ & 647s  \\ \hline
$[-0.05, -0.025] \times [0.025, 0.05]$ & $\|r_3\|_{\infty} \le 0.32m$ & 3534s  \\ \hline
$[-0.025, 0] \times [0.025, 0.05]$ & $\|r_3\|_{\infty} \le 0.32m$ & 2491s  \\ \hline
$[0, 0.025] \times [0.025, 0.05]$ & $\|r_3\|_{\infty} \le 0.32m$ & 2142s  \\ \hline
$[0.025, 0.05] \times [0.025, 0.05]$ & $\|r_3\|_{\infty} \le 0.32m$ & 1090s  \\ \hline
\end{tabular}
\caption{Verisig+Flow* verification times (in seconds) for different
  initial conditions of the quadrotor case study. All properties were
  verified. Note that $r_3 = [p_x^r, p_y^r, p_z^r]$.}
\label{tab:quad_cs}
\end{table}


Similar to the Moutain Car case study, we split the initial condition
into smaller subsets and verified the property for each subset. The
verification times of Verisig+Flow* for each subset are shown in
Table~\ref{tab:quad_cs}. Most cases take less than 30 minutes to
verify, which is still acceptable given that the computation is
performed offline. Note that this verification task is harder than the
Mountain Car one not because of the larger dimension of the state
space but rather because of the discrete nature of the DNN
outputs. This means that Verisig effectively needs to enumerate and
verify all possible paths from the initial condition. Computing all
paths is computationally expensive since the number of paths could
grow exponentially with the length of the scenario (set to 30 steps in
this case study). One approach to reduce the computation time would be
to use the Markov property of dynamical systems and not verify states
that have been reached and verified previously. We plan to explore
this idea as part of future work.

Thus, we have shown that Verisig can be used to verify interesting
properties in different and challenging domains. The properties
verified include both safety and liveness properties, and the plant
models are nonlinear systems specified in either discrete or
continuous time. The next section shows that Verisig+Flow* also scales
well to larger DNNs and is competitive with other approaches even for
verification of DNN properties in isolation.

